Particularity

We describe a design principle for adaptive systems under which adaptation is driven by particular challenges that the environment poses, as opposed to average or otherwise aggregated measures of performance over many challenges. We trace the development of this "particularity" approach from the use of lexicase selection in genetic programming to "particularist" approaches to other forms of machine learning and to the design of adaptive systems more generally.

==> hidden_lexfigs/hardMazes.tex <==
\newsavebox{\largestimage}
\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.55\textwidth}
         \centering
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1.5,xscale=1.5]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp4919490977130325] 
\draw   (110.33,99.33) -- (325,99.33) -- (325,195.67) -- (110.33,195.67) -- cycle ;
%Shape: Circle [id:dp9887019347294541] 
\draw   (123.67,111.33) .. controls (123.67,109.31) and (125.31,107.67) .. (127.33,107.67) .. controls (129.36,107.67) and (131,109.31) .. (131,111.33) .. controls (131,113.36) and (129.36,115) .. (127.33,115) .. controls (125.31,115) and (123.67,113.36) .. (123.67,111.33) -- cycle ;
%Straight Lines [id:da5357263133899859] 
\draw    (191.33,99) -- (160,126) ;
%Straight Lines [id:da45987057756590666] 
\draw    (147.67,148.67) -- (286.33,196) ;
%Straight Lines [id:da7852541457857296] 
\draw    (255.67,99) -- (210.33,133.67) ;
%Straight Lines [id:da3850033125849259] 
\draw    (308.33,99.67) -- (266.67,143) ;
%Straight Lines [id:da22447890927809877] 
\draw    (186.67,130.67) -- (206.33,169) ;
%Straight Lines [id:da8873570825982717] 
\draw    (242.33,143) -- (272,191) ;
%Straight Lines [id:da7845558014349576] 
\draw    (283.67,161.67) -- (311.67,196) ;
%Shape: Circle [id:dp4911251469948623] 
\draw   (305.5,170.75) .. controls (305.5,169.65) and (306.4,168.75) .. (307.5,168.75) .. controls (308.6,168.75) and (309.5,169.65) .. (309.5,170.75) .. controls (309.5,171.85) and (308.6,172.75) .. (307.5,172.75) .. controls (306.4,172.75) and (305.5,171.85) .. (305.5,170.75) -- cycle ;
\end{tikzpicture}
         \caption{Medium Map}
         \label{fig:MediumMap}\hspace*{-2.9em}
     \end{subfigure}
     \hfill
     \savebox{\largestimage}{
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,510); %set diagram left start at 0, and has height of 510

%Shape: Polygon [id:ds31414295104263146] 
\draw   (299.67,227) -- (309.67,432.67) -- (108.33,437) -- (104,227.67) -- (144,224) -- cycle ;
%Straight Lines [id:da3950419722736951] 
\draw    (105,271.33) -- (162,277.33) ;
%Straight Lines [id:da08924819695350994] 
\draw    (162,277.33) -- (243,250.67) ;
%Straight Lines [id:da11251252107495513] 
\draw    (162,277.33) -- (161.33,388.67) ;
%Straight Lines [id:da42059545299212653] 
\draw    (105.33,302) -- (136,349.33) ;
%Straight Lines [id:da13516287039153307] 
\draw    (161.67,333) -- (269.33,393.67) ;
%Straight Lines [id:da9972492114133158] 
\draw    (193.67,317.33) -- (307.33,377) ;
%Straight Lines [id:da5025799709706835] 
\draw    (216.67,396) -- (184.33,435.67) ;
%Shape: Circle [id:dp7666213194094769] 
\draw   (134,417.83) .. controls (134,414.98) and (136.31,412.67) .. (139.17,412.67) .. controls (142.02,412.67) and (144.33,414.98) .. (144.33,417.83) .. controls (144.33,420.69) and (142.02,423) .. (139.17,423) .. controls (136.31,423) and (134,420.69) .. (134,417.83) -- cycle ;
%Shape: Circle [id:dp28786302234420846] 
\draw   (132.33,240.33) .. controls (132.33,239.23) and (133.23,238.33) .. (134.33,238.33) .. controls (135.44,238.33) and (136.33,239.23) .. (136.33,240.33) .. controls (136.33,241.44) and (135.44,242.33) .. (134.33,242.33) .. controls (133.23,242.33) and (132.33,241.44) .. (132.33,240.33) -- cycle ;
\end{tikzpicture}
}
     \begin{subfigure}[b]{0.42\textwidth}
         \centering
         \usebox{\largestimage}
         \caption{Hard Map}
         \label{fig:hardmaze}
         
     \end{subfigure}
        \caption{Two deceptive mazes, adapted from \citep{lehman_abandoning_2011}. In both maps, the large circle is the starting point of the robot and the small circle represents the goal. Both maps are deceptive in the sense that the path that minimizes euclidean distance to the goal will get stuck at local optima.}
        \label{fig:mazes}
\end{figure*}
